Universal asymptotic clone size distribution for general population growth

Deterministically growing (wild-type) populations which seed stochastically developing mutant clones have found an expanding number of applications from microbial populations to cancer. The special case of exponential wild-type population growth, usually termed the Luria-Delbr\"uck or Lea-Coulson model, is often assumed but seldom realistic. In this article we generalise this model to different types of wild-type population growth, with mutants evolving as a birth-death branching process. Our focus is on the size distribution of clones - that is the number of progeny of a founder mutant - which can be mapped to the total number of mutants. Exact expressions are derived for exponential, power-law and logistic population growth. Additionally for a large class of population growth we prove that the long time limit of the clone size distribution has a general two-parameter form, whose tail decays as a power-law. Considering metastases in cancer as the mutant clones, upon analysing a data-set of their size distribution, we indeed find that a power-law tail is more likely than an exponential one.

==> cancer4_bmb.tex <==
@article{Angerer:2001,
author = {Angerer, Wolfgang P},
journal = {Journal of Mathematical Biology},
number = {2},
pages = {145--174},
title = {{An explicit representation of the Luria-Delbr\"{u}ck Distribution}},
volume = {42},
year = {2001}
}
@article{Anglani:2007,
archivePrefix = {arXiv},
arxivId = {arXiv:math/0702010v1},
author = {Anglani, Roberto and Barile, Margherita},
eprint = {0702010v1},
primaryClass = {arXiv:math},
title = {{Factorials as sums}},
year = {2007}
}
@article{Antal:2011,
author = {Antal, T and Krapivsky, P L},
journal = {J. Stat. Mech. P08018},
title = {{Exact solution of a two-type branching process: models of tumor progression}},
year = {2011}
}
@article{Antal:2010,
author = {Antal, Tibor and Krapivsky, P L},
issn = {1742-5468},
journal = {J. Stat. Mech. P07028},
number = {7},
title = {{Exact solution of a two-type branching process: clone size distribution in cell division kinetics}},
year = {2010}
}
@article{Araten:2005,
abstract = {The mutation rate (mu) is a key biological feature of somatic cells that determines risk for malignant transformation, and it has been exceedingly difficult to measure in human cells. For this purpose, a potential sentinel is the X-linked PIG-A gene, because its inactivation causes lack of glycosylphosphatidylinositol-linked membrane proteins. We previously found that the frequency (f) of PIG-A mutant cells can be measured accurately by flow cytometry, even when f is very low. Here we measure both f and mu by culturing B-lymphoblastoid cell lines and first eliminating preexisting PIG-A mutants by flow sorting. After expansion in culture, the frequency of new mutants is determined by flow cytometry using antibodies specific for glycosylphosphatidylinositol-linked proteins (e.g., CD48, CD55, and CD59). The mutation rate is then calculated by the formula mu = f/d, where d is the number of cell divisions occurring in culture. The mean mu in cells from normal donors was 10.6 x 10(-7) mutations per cell division (range 2.4 to 29.6 x 10(-7)). The mean mu was elevated >30-fold in cells from patients with Fanconi anemia (P < 0.0001), and mu varied widely in ataxia-telangiectasia with a mean 4-fold elevation (P = 0.002). In contrast, mu was not significantly different from normal in cells from patients with Nijmegen breakage syndrome. Differences in mu could not be attributed to variations in plating efficiency. The mutation rate in man can now be measured routinely in B-lymphoblastoid cell lines, and it is elevated in cancer predisposition syndromes. This system should be useful in evaluating cancer risk and in the design of preventive strategies.},
author = {Araten, David J. and Golde, David W. and Zhang, Rong H. and Thaler, Howard T. and Gargiulo, Lucia and Notaro, Rosario and Luzzatto, Lucio},
doi = {10.1158/0008-5472.CAN-04-1198},
issn = {00085472},
journal = {Cancer Research},
number = {18},
pages = {8111--8117},
pmid = {16166284},
title = {{A quantitative measurement of the human somatic mutation rate}},
volume = {65},
year = {2005}
}
@article{Armitage:1952,
author = {Armitage, P.},
journal = {Journal of Royal Statistical Society B},
number = {1},
title = {{The statistical theory of bacterial populations subject to mutations}},
year = {1952}
}
@book{Athreya:2004,
author = {Athreya, K B and Ney, P E},
publisher = {Dover Publications},
title = {{Branching Processes}},
year = {2004}
}
@book{Bailey:1964,
author = {Bailey, Norman T J},
publisher = {John Wiley \& Sons, Inc},
title = {{The elements of stochastic processes with applications to the natural sciences}},
year = {1964}
}
@book{Bartlett:1955,
author = {Bartlett, M.S.},
edition = {3rd},
publisher = {Cambridge University Press},
title = {{An Introduction to Stochastic Processes}},
year = {1955}
}
@book{Burnham:1998,
author = {Burnham, K.P. and Anderson, D.R. },
publisher = {Springer},
title = {{ Model selection and inference: a practical information-theoretic approach}},
year = {1998}
}
@book{Bingham:1987,
author = {Bingham, N.H. and Goldie, C.M. and Teugels, J.L.},
publisher = {Cambridge University Press},
title = {{Regular Variation}},
year = {1987}
}
@article{Bozic:2014,
author = {Bozic, Ivana and Nowak, Martin},
journal = {Proceedings of the National Academy of Science USA},
number = {45},
title = {{Timing and heterogeneity of mutations associated with drug resistance in metastatic cancers}},
volume = {111},
year = {2014}
}
@article{Bozic:2013,
abstract = {In solid tumors, targeted treatments can lead to dramatic regressions, but responses are often short-lived because resistant cancer cells arise. The major strategy proposed for overcoming resistance is combination therapy. We present a mathematical model describing the evolutionary dynamics of lesions in response to treatment. We first studied 20 melanoma patients receiving vemurafenib. We then applied our model to an independent set of pancreatic, colorectal, and melanoma cancer patients with metastatic disease. We find that dual therapy results in long-term disease control for most patients, if there are no single mutations that cause cross-resistance to both drugs; in patients with large disease burden, triple therapy is needed. We also find that simultaneous therapy with two drugs is much more effective than sequential therapy. Our results provide realistic expectations for the efficacy of new drug combinations and inform the design of trials for new cancer therapeutics. DOI:http://dx.doi.org/10.7554/eLife.00747.001.},
author = {Bozic, Ivana and Reiter, Johannes G. and Allen, Benjamin and Antal, Tibor and Chatterjee, Krishnendu and Shah, Preya and Moon, Yo Sup and Yaqubie, Amin and Kelly, Nicole and Le, Dung T. and Lipson, Evan J. and Chapman, Paul B. and Diaz, Luis A. and Vogelstein, Bert and Nowak, Martin A.},
file = {:C$\backslash$:/Users/Michael/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Bozic et al. - 2013 - Evolutionary dynamics of cancer in response to targeted combination therapy.pdf:pdf},
isbn = {2050-084X (Electronic)},
issn = {2050084X},
journal = {eLife: e00747},
number = {2},
pmid = {23805382},
title = {{Evolutionary dynamics of cancer in response to targeted combination therapy}},
year = {2013}
}
@article{Clauset:2009,
abstract = {Power-law distributions occur in many situations of scientific interest and have significant consequences for our understanding of natural and man-made phenomena. Unfortunately, the detection and characterization of power laws is complicated by the large fluctuations that occur in the tail of the distribution—the part of the distribution representing large but rare events—and by the difficulty of identifying the range over which power-law behavior holds. Commonly used methods for analyzing power-law data, such as least-squares fitting, can produce substantially inaccurate estimates of parameters for power-law distributions, and even in cases where such methods return accurate answers they are still unsatisfactory because they give no indication of whether the data obey a power law at all. Here we present a principled statistical framework for discerning and quantifying power-law behavior in empirical data. Our approach combines maximum-likelihood fitting methods with goodness-of-fit tests based on the Kolmogorov–Smirnov (KS) statistic and likelihood ratios. We evaluate the effectiveness of the approach with tests on synthetic data and give critical comparisons to previous approaches. We also apply the proposed methods to twenty-four real-world data sets from a range of different disciplines, each of which has been conjectured to follow a power-law distribution. In some cases we find these conjectures to be consistent with the data, while in others the power law is ruled out.},
author = {Clauset, A and Shalizi, C R and Newman, M E J},
journal = {SIAM Review},
keywords = {Clauset:2009},
mendeley-tags = {Clauset:2009},
pages = {661--703},
title = {{Power-law distributions in empirical data}},
volume = {51},
year = {2009}
}
@article{Clayton:2007aa,
annote = {10.1038/nature05574},
author = {Clayton, Elizabeth and Doupe, David P and Klein, Allon M and Winton, Douglas J and Simons, Benjamin D and Jones, Philip H},
isbn = {0028-0836},
journal = {Nature},
number = {7132},
pages = {185--189},
title = {{A single type of progenitor cell maintains normal epidermis}},
url = {http://dx.doi.org/10.1038/nature05574},
volume = {446},
year = {2007}
}
@article{Crump:1974,
author = {Crump, Kenny S and Hoel, David G},
doi = {10.1093/biomet/61.2.237},
issn = {1464-3510},
journal = {Biometrika},
month = aug,
number = {2},
pages = {237--252},
publisher = {Oxford University Press},
title = {{Mathematical models for estimating mutation rates in cell populations}},
volume = {61},
year = {1974}
}
@book{deHaan:2006,
abstract = {This treatment of extreme value theory is unique in book literature in that it focuses on some beautiful theoretical results along with applications. All the main topics covering the heart of the subject are introduced to the reader in a systematic fashion so that in the final chapter even the most recent developments in the theory can be understood.$\backslash$n$\backslash$nKey to the presentation is the concentration on the probabilistic and statistical aspects of extreme values without major emphasis on such related topics as regular variation, point processes, empirical distribution functions, and Brownian motion.$\backslash$n$\backslash$nThe work is an excellent introduction to extreme value theory at the graduate level, requiring only some mathematical maturity.},
author = {de Haan, Laurens and Ferreira, Ana},
booktitle = {Analysis},
doi = {10.1007/0-387-33477-7},
isbn = {0387239464},
publisher = {Springer},
title = {{Extreme Value Theory: An Introduction}},
year = {2006}
}

@article{Dewanji:2005,
author = {Dewanji, A and Luebeck, E G and Moolgavkar, S H},
issn = {0025-5564},
journal = {Mathematical Biosciences},
keywords = {Mutant clones},
number = {2},
pages = {140--152},
title = {{A generalized Luria-Delbr\"{u}ck model}},
volume = {197},
year = {2005}
}
@article{Dewanji:2011,
author = {Dewanji, Anup and Jeon, Jihyoun and Mexa, Rafael and Luebeck, E Georg},
journal = {PLoS Computational Biology},
number = {10},
title = {{Number and size distribution of colorectal adenomas under the multistage clonal expansion model of cancer}},
volume = {7},
year = {2011}
}


@article{Diaz:2012,
abstract = {Colorectal tumours that are wild type for KRAS are often sensitive to EGFR blockade, but almost always develop resistance within several months of initiating therapy. The mechanisms underlying this acquired resistance to anti-EGFR antibodies are largely unknown. This situation is in marked contrast to that of small-molecule targeted agents, such as inhibitors of ABL, EGFR, BRAF and MEK, in which mutations in the genes encoding the protein targets render the tumours resistant to the effects of the drugs. The simplest hypothesis to account for the development of resistance to EGFR blockade is that rare cells with KRAS mutations pre-exist at low levels in tumours with ostensibly wild-type KRAS genes. Although this hypothesis would seem readily testable, there is no evidence in pre-clinical models to support it, nor is there data from patients. To test this hypothesis, we determined whether mutant KRAS DNA could be detected in the circulation of 28 patients receiving monotherapy with panitumumab, a therapeutic anti-EGFR antibody. We found that 9 out of 24 (38\%) patients whose tumours were initially KRAS wild type developed detectable mutations in KRAS in their sera, three of which developed multiple different KRAS mutations. The appearance of these mutations was very consistent, generally occurring between 5 and 6 months following treatment. Mathematical modelling indicated that the mutations were present in expanded subclones before the initiation of panitumumab treatment. These results suggest that the emergence of KRAS mutations is a mediator of acquired resistance to EGFR blockade and that these mutations can be detected in a non-invasive manner. They explain why solid tumours develop resistance to targeted therapies in a highly reproducible fashion.},
author = {{Diaz Jr}, Luis A. and Williams, Richard T. and Wu, Jian and Kinde, Isaac and Hecht, J. Randolph and Berlin, Jordan and Allen, Benjamin and Bozic, Ivana and Reiter, Johannes G. and Nowak, Martin A. and Kinzler, Kenneth W. and Oliner, Kelly S. and Vogelstein, Bert},
isbn = {1476-4687 (Electronic)$\backslash$r0028-0836 (Linking)},
issn = {0028-0836},
journal = {Nature},
pages = {537--540},
volume = {486},
pmid = {22722843},
title = {{The molecular evolution of acquired resistance to targeted EGFR blockade in colorectal cancers}},
year = {2012}
}
@article{Durrett2010,
abstract = {Inspired by previous work of Iwasa et al. (2006) and Haeno et al. (2007), we consider an exponentially growing population of cancerous cells that will evolve resistance to treatment after one mutation or display a disease phenotype after two or more mutations. We prove results about the distribution of the first time when k mutations have accumulated in some cell, and about the growth of the number of type-k cells. We show that our results can be used to derive the previous results about a tumor grown to a fixed size. © 2009 Elsevier Inc. All rights reserved.},
author = {Durrett, Richard and Moseley, Stephen},
doi = {10.1016/j.tpb.2009.10.008},
file = {:C$\backslash$:/Users/Michael/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Durrett, Moseley - 2010 - Evolution of resistance and progression to disease during clonal expansion of cancer.pdf:pdf},
issn = {00405809},
journal = {Theoretical Population Biology},
keywords = {Branching process,Cancer models,Moran model,Waiting times},
number = {1},
pages = {42--48},
pmid = {19896491},
publisher = {Elsevier Inc.},
title = {{Evolution of resistance and progression to disease during clonal expansion of cancer}},
url = {http://dx.doi.org/10.1016/j.tpb.2009.10.008},
volume = {77},
year = {2010}
}
@article{Durrett:2010,
author = {Durrett, Richard and Moseley, Stephen},
journal = {Theoretical Population Biology},
number = {1},
pages = {42--48},
title = {{Evolution of resistance and progression to disease during clonal expansion of cancer}},
volume = {77},
year = {2010}
}
@book{Durrett:1996,
author = {Durrett, Rick},
publisher = {Cambridge University Press},
edition = {4th},
series = {Cambridge Series in Statistical and Probabilistic Mathematics},
title = {{Probability: Theory and Examples}},
year = {1996}
}
@book{Durrett:2015,
author = {Durrett, Rick},
publisher = {Springer International Publishing},
edition = {1},
series = {Stochastics in Biological Systems},
title = {{Branching Process Models of Cancer}},
year = {2015}
}
@book{Feller:1968,
abstract = {Capter IV discusses the inclusion-exclusion principle, and the occupancy problem, ie., it calculates the probability that m slots will be empty, after putting r balls among n slots. Moreover, it approximates this probability with the poisson distribution.},
author = {Feller, W},
booktitle = {Wiley},
doi = {10.2307/1266435},
edition = {2nd},
isbn = {0471257087},
issn = {00401706},
pages = {509},
title = {{An Introduction to Probability Theory and Its Applications}},
volume = {2},
year = {1968}
}
@book{Flajolet:2009,
author = {Flajolet, Philippe and Sedgewick, Robert},
isbn = {978-0-521-89806-5},
pages = {xiv+810},
publisher = {Cambridge University Press, Cambridge},
title = {{Analytic Combinatorics}},
year = {2009}
}
@misc{Flajolet1995,
abstract = {High order differences of simple number sequences may be analysed asymptotically by means of integral representations, residue calculus, and contour integration. This technique, akin to Mellin transform asymptotics, is put in perspective and illustrated by means of several examples related to combinatorics and the analysis of algorithms like digital tries, digital search trees, quadtrees, and distributed leader election.},
author = {Flajolet, Philippe and Sedgewick, Robert},
booktitle = {Theoretical Computer Science},
issn = {03043975},
number = {1-2},
pages = {101--124},
title = {{Mellin transforms and asymptotics: Finite differences and Rice's integrals}},
volume = {144},
year = {1995}
}
@article{Foo:2014,
author = {Foo, Jasmine and Michor, Franziska},
journal = {Journal of Theoretical Biology},
title = {{Evolution of acquired resistance to anti-cancer therapy}},
volume = {355},
pages = {10--20},
year = {2014}
}
@misc{Gerlee:2013,
abstract = {In this article, we will trace the historical development of tumor growth laws, which in a quantitative fashion describe the increase in tumor mass/volume over time. These models are usually formulated in terms of differential equations that relate the growth rate of the tumor to its current state and range from the simple one-parameter exponential growth model to more advanced models that contain a large number of parameters. Understanding the assumptions and consequences of such models is important, as they often underpin more complex models of tumor growth. The conclusion of this brief survey is that although much improvement has occurred over the last century, more effort and new models are required if we are to understand the intricacies of tumor growth.},
archivePrefix = {arXiv},
arxivId = {1209.3170},
author = {Gerlee, Philip},
booktitle = {Cancer Research},
doi = {10.1158/0008-5472.CAN-12-4355},
eprint = {1209.3170},
issn = {00085472},
number = {8},
pages = {2407--2411},
pmid = {23393201},
title = {{The model muddle: In search of tumor growth laws}},
volume = {73},
year = {2013}
}
@article{Goldie:1995,
author = {Goldie, Charles M},
journal = {Journal of Applied Probability},
number = {3},
pages = {840--841},
title = {{Asymptotics of the \{L\}uria-\{D\}elbr\"{u}ck Distribution}},
volume = {32},
year = {1995}
}
@book{Grimmett:1992,
author = {{Grimmett, G.R.;Stirzaker}, D.R.},
edition = {2nd},
publisher = {Oxford University Press},
title = {{Probability and Random Processes}},
year = {1992}
}
@article{Hanin:2006,
abstract = {A stochastic entirely mechanistic model of metastatic progression of cancer is developed. Based on this model the joint conditional distribution of the ordered sizes of detectable metastases given their number, n, is computed. It is shown that this distribution coincides with the joint distribution of order statistics for a random sample of size n derived from some probability distribution, and a formula for the latter is obtained. This formula is specialized for the case of exponentially growing primary and secondary tumors and exponentially distributed metastasis promotion times, and identifiability of model parameters is ascertained. These results allow for estimation of the natural history of cancer. As an example, it is estimated for a breast cancer patient with 31 bone metastases of known sizes. The proposed model for the sizes of detectable metastases provided an excellent fit to these data. ?? 2006 Elsevier Ltd. All rights reserved.},
author = {Hanin, Leonid and Rose, Jason and Zaider, Marco},
issn = {00225193},
journal = {Journal of Theoretical Biology},
keywords = {Cancer natural history,Metastasis,Model identifiability,Poisson process,Primary tumor},
number = {3},
pages = {407--417},
pmid = {16930629},
title = {{A stochastic model for the sizes of detectable metastases}},
volume = {243},
year = {2006}
}
@book{Harris:1963,
address = {Berlin, G\{\"{o}\}ttingen, Heidelberg},
author = {Harris, Theodore Edward},
publisher = {Springer},
series = {Die Grundlehren der mathematischen Wissenschaften},
title = {{The theory of branching processes}},
url = {http://opac.inria.fr/record=b1081408},
year = {1963}
}
@article{Houchmandzadeh:2015,
author = {Houchmandzadeh, Bahram},
journal = {Physical Review E, 012719},
title = {{General formulation of Luria-Delbr\"{u}ck distribution of the number of mutants}},
volume = {92},
year = {2015}
}
@article{Hudson:1971,
abstract = {During the last few years, several authors have devoted attention to both old and new methods of making inferences from likelihood functions. In this paper we study the properties of interval estimates which are obtained by drawing a horizontal line across the graph of the likelihood function. An exact evaluation is reported for one case of positive and one of negative binomial sampling, with parameter $\theta$. The attained confidence coefficient $\alpha$($\theta$) is graphed over 0 ⩽ $\theta$ ⩽ 1 for these two cases. A brief look is taken at intervals obtained when the random variable is continuous.},
author = {Hudson, D J},
isbn = {00359246},
journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
number = {2},
pages = {256--262},
title = {{Interval estimation from the likelihood function}},
volume = {33},
year = {1971}
}
@article{Iwasa:2006,
author = {Iwasa, Yoh and Nowak, Martin A and Michor, Franziska},
journal = {Genetics},
number = {4},
pages = {2557--2566},
title = {{Evolution of resistance during clonal expansion}},
volume = {172},
year = {2006}
}
@article{Janson:2006,
author = {Janson, Svante},
journal = {Probability Theory and Related Fields},
number = {3},
pages = {417--452},
title = {{Limit theorems for triangular urn schemes}},
volume = {134},
year = {2006}
}
@article{Jeon:2008,
abstract = {We derive mathematical expressions for the size distribution of screen-detectable pre-malignant lesions, both conditional and unconditional on no prior detection of cancer in the tissue of interest, based on a general multistage clonal expansion model of carcinogenesis. We apply these expressions to simulate the natural history of colorectal cancer and to evaluate the effect of a screen for adenomatous polyps and concomitant intervention on cancer risk. Our approach allows the efficient simulation of multiple screens and interventions and determination of the optimal timing of the screens. We further demonstrate the utility of our approach by computing the benefits of up to two colonoscopies on the lifetime risk of colorectal cancer. © 2008 Elsevier Inc. All rights reserved.},
author = {Jeon, Jihyoun and Meza, Rafael and Moolgavkar, Suresh H. and Luebeck, E. Georg},
isbn = {0025-5564},
issn = {00255564},
journal = {Mathematical Biosciences},
keywords = {Cancer screening,Colonoscopy,Multistage carcinogenesis,Pre-malignant lesion},
number = {1},
pages = {56--70},
pmid = {18374369},
title = {{Evaluation of screening strategies for pre-malignant lesions using a biomathematical approach}},
volume = {213},
year = {2008}
}
@book{Karlin:1975,
author = {Karlin, Samuel and Taylor, Howard M},
publisher = {New York - San Francisco - London: Academic Press, Inc., a subsidiary of Harcourt Brace Jovanovich, Publishers. XVI},
title = {{A first course in stochastic processes}},
year = {1975}
}
@book{Karlin:1981,
author = {Karlin, Samuel and Taylor, Howard M},
publisher = {New York - San Francisco - London: Academic Press, Inc., a subsidiary of Harcourt Brace Jovanovich, Publishers. XVI},
title = {{A Second Course in Stochastic Processes}},
year = {1981}
}

@book{Karlin:1998,
abstract = {Conditional Probability and Conditional Expectation Markov Chains: Introduction The Long Run Behavior of Markov Chains Poisson Processes Continuous Time Markov Chains Renewal Phenomena Brownian Motion and Related Processes Queueing Systems},
author = {Karlin, Samuel and Taylor, Howard M.},
edition = {3rd},
isbn = {978-0-12-684887-8},
publisher = {Academic Press Inc.},
title = {{An Introduction to Stochastic Modeling}},
year = {1998}
}
@article{Keller:2015,
author = {Keller, Peter and Antal, Tibor},
file = {:C$\backslash$:/Users/Michael/Google Drive/tumor/luria-delbruck/Keller15.pdf:pdf},
issn = {1742-5468},
journal = {J. Stat. Mech. P01011},
number = {1},
publisher = {IOP Publishing},
title = {{Mutant number distribution in an exponentially growing population}},
year = {2015}
}
@article{Kemp:1994,
author = {Kemp, Adrienne W},
journal = {Journal of Applied Probability},
number = {3},
pages = {822--828},
title = {{Comments on the Luria-Delbr\"{u}ck Distribution}},
volume = {31},
year = {1994}
}
@article{Kendal:1988,
author = {Kendal, Wayne S and Frost, Philip},
journal = {CANCER RESEARCH},
pages = {1060--1065},
title = {{Pitfalls and Practice of \{L\}uria-\{D\}elbr\"{u}ck Fluctuation Analysis: A Review}},
volume = {48},
year = {1988}
}
@article{Kendall:1948,
author = {Kendall, David G},
file = {:C$\backslash$:/Users/Michael/Google Drive/tumor/others/Kendall48.pdf:pdf},
journal = {Biometrika},
number = {1/2},
pages = {6--15},
title = {{On some modes of population growth leading to R. A. Fisher's logarithmic series distribution}},
volume = {35},
year = {1948}
}
@article{Kendall:1960,
author = {Kendall, David G},
issn = {0006-3444},
journal = {Biometrika},
pages = {13--21},
title = {{Birth-and-death processes, and the theory of carcinogenesis}},
volume = {47},
year = {1960}
}
@article{Kessler:2015,
archivePrefix = {arXiv},
author = {Kessler, D.A. and Levine, H.},
journal = {Journal of Statistical Physics},
keywords = {Condensed Matter - Statistical Mechanics,Quantitative Biology - Populations and Evolution},
month = apr,
number = {4},
pages = {783--805},
primaryClass = {q-bio.PE},
title = {{Scaling solution in the large population limit of the general asymmetric stochastic Luria–Delbr\"{u}ck evolution process}},
volume = {158,},
year = {2015}
}
@article{Kessler:2014,
abstract = {The issue of resistance to targeted drug therapy is of pressing concern, as it constitutes a major barrier to progress in managing cancer. One important aspect is the role of stochasticity in determining the nature of the patient response. We examine two particular experiments. The first measured the maximal response of melanoma to targeted therapy before the resistance causes the tumor to progress. We analyze the data in the context of a Delbruck-Luria type scheme, wherein the continued growth of preexistent resistant cells are responsible for progression. We show that, aside from a finite fraction of resistant cell-free patients, the maximal response in such a scenario would be quite uniform. To achieve the measured variability, one is necessarily led to assume a wide variation from patient to patient of the sensitive cells' response to the therapy. The second experiment is an in vitro system of multiple myeloma cells. When subject to a spatial gradient of a chemotherapeutic agent, the cells in the middle of the system acquire resistance on a rapid (two-week) timescale. This finding points to the potential important role of cell-to-cell differences, due to differing local environments, in addition to the patient-to-patient differences encountered in the first part. See all articles in this Cancer Research section, "Physics in Cancer Research."},
author = {Kessler, David A and Austin, Robert H and Levine, Herbert},
issn = {1538-7445},
journal = {Cancer research},
keywords = {Antineoplastic Agents,Antineoplastic Agents: therapeutic use,Disease Progression,Drug Resistance,Humans,Individuality,Neoplasm,Neoplasm: physiology,Neoplasms,Neoplasms: drug therapy},
number = {17},
pages = {4663--70},
pmid = {25183790},
title = {{Resistance to chemotherapy: patient variability and cellular heterogeneity.}},
volume = {74},
year = {2014}
}
@article{Kessler:2013,
author = {Kessler, David A and Levine, Herbert},
journal = {Proceedings of the national Academy of Science USA},
number = {29},
pages = {11682--11687},
title = {{Large population solution of the stochastic \{L\}uria-\{D\}elbr\"{u}ck evolution model}},
volume = {110},
year = {2013}
}
@article{Kimmel:1994,
author = {Kimmel, Marek and Axelrod, David E},
journal = {Mutation Research},
pages = {45--60},
title = {{Fluctuation test for two-stage mutations: application to gene amplification}},
volume = {306},
year = {1994}
}
@article{Koch:1982,
author = {Koch, Arthur L},
journal = {Mutation Research},
pages = {129--143},
title = {{Mutation and growth rates from \{L\}uria-\{D\}elbr\"{u}ck fluctuation tests}},
volume = {95},
year = {1982}
}
@article{Komarova:2006,
author = {Komarova, Natalia},
journal = {Journal of Theoretical Biology},
pages = {351--366},
title = {{Stochastic modeling of drug resistance in cancer}},
volume = {239},
year = {2006}
}
@article{Komarova:2007,
author = {Komarova, Natalia L and Wu, Lin and Baldi, Pierre},
journal = {Mathematical Biosciences},
pages = {253--290},
title = {{The fixed-size Luria-Delbr\"{u}ck model with nonzero death rate}},
volume = {210},
year = {2007}
}

@article{Krapivsky:2001,
abstract = {The organizational development of growing random networks is investigated. These growing networks are built by adding nodes successively and linking each to an earlier node of degree k with attachment probability A\_k. When A\_k grows slower than linearly with k, the number of nodes with k links, N\_k(t), decays faster than a power-law in k, while for A\_k growing faster than linearly in k, a single node emerges which connects to nearly all other nodes. When A\_k is asymptotically linear, N\_k(t) tk\^{}\{-nu\}, with nu dependent on details of the attachment probability, but in the range 2<nu<infty. The combined age and degree distribution of nodes shows that old nodes typically have a large degree. There is also a significant correlation in the degrees of neighboring nodes, so that nodes of similar degree are more likely to be connected. The size distributions of the in-components and out-components of the network with respect to a given node -- namely, its "descendants" and "ancestors" -- are also determined. The in-component exhibits a robust s\^{}\{-2\} power-law tail, where s is the component size. The out component has a typical size of order ln t and it provides basic insights about the genealogy of the network.},
archivePrefix = {arXiv},
author = {Krapivsky, P. L. and Redner, S.},
isbn = {1539-3755},
issn = {1063-651X},
journal = {Physical Review E 1--066123},
number = {6},
pmid = {11415189},
primaryClass = {cond-mat},
title = {{Organization of Growing Random Networks}},
volume = {63},
year = {2001}
}


@article{Lea:1949,
author = {Lea, D E and Coulson, C A},
issn = {0022-1333},
journal = {Journal of Genetics},
number = {3},
pages = {264--285},
publisher = {Springer India},
title = {{The distribution of the numbers of mutants in bacterial populations}},
volume = {49},
year = {1949}
}
@article{Luria:1943,
author = {Luria, S E and Delbr\"{u}ck, M},
journal = {Genetics},
number = {6},
pages = {491--511},
title = {{Mutations of bacteria from virus sensitivity to virus resistance}},
volume = {48},
year = {1943}
}
@article{Ma:1992,
author = {Ma, W T and Sandri, G Vh. and Sarkar, S},
journal = {Journal of Applied Probability},
number = {2},
pages = {255--267},
title = {{Analysis of the \{L\}uria-\{D\}elbr\"{u}ck Distribution using discrete convolution powers}},
volume = {29},
year = {1992}
}
@article{Mandelbrot:1974,
abstract = {Luria and Delbr\{\"{u}\}ck (1943) have observed that, in old cultures of bacteria that have mutated at random,
the distribution of the number of mutants is extremely long-tailed. In this note, this distribution will be derived (for
the first time) exactly and explicitly. The rates of mutation will be allowed to be either positive or infinitesimal,
and the rate of growth for mutants will be allowed to be either equal, greater or smaller than for non-mutants. Under
the realistic limit condition of a very low mutation rate, the number of mutants is shown to be a stable-L\{\'{e}\}vy
(sometimes called "Pareto L\{\'{e}\}vy") random variable, of maximum skewness $\beta$, whose exponent $\alpha$ is essentially the ratio of
the growth rates of non-mutants and of mutants. Thus, the probability of the number of mutants exceeding the very large
value m is proportional to m- $\alpha$ - 1 (a behavior sometimes referred to as "asymptotically Paretian" or "hyperbolic"). The
unequal growth rate cases $\alpha$ ≠ 1 are solved for the first time. In the $\alpha$ = 1 case, a result of Lea and Coulson is
rederived, interpreted, and generalized. Various paradoxes involving divergent moments that were encountered in earlier
approaches are either absent or fully explainable. The mathematical techniques used being standard, they will not be
described in detail, so this note will be primarily a collection of results. However, the justification for deriving
them lies in their use in biology, and the mathematically unexperienced biologists may be unfamiliar with the tools
used. They may wish for more details of calculations, more explanations and Figures. To satisfy their needs, a report
available from the author upon request has been prepared. It will be referred to as Part II.},
author = {Mandelbrot, Benoit},
issn = {00219002},
journal = {Journal of Applied Probability},
number = {3},
pages = {pp. 437--444},
publisher = {Applied Probability Trust},
title = {{A Population Birth-and-Mutation Process, I: Explicit Distributions for the Number of Mutants in an Old Culture of Bacteria}},
url = {http://www.jstor.org/stable/3212688},
volume = {11},
year = {1974}
}
@article{Mehlen:2006,
abstract = {The metastatic process is highly inefficient--very few of the many cells that migrate from the primary tumour successfully colonize distant sites. One proposed mechanism to explain this inefficiency is provided by the cancer stem cell model, which hypothesizes that micrometastases can only be established by tumour stem cells, which are few in number. However, recent in vitro and in vivo observations indicate that apoptosis is an important process regulating metastasis. Here we stress that the inhibition of cell death, apart from its extensively described function in primary tumour development, is a crucial characteristic of metastatic cancer cells.},
author = {Mehlen, Patrick and Puisieux, Alain},
doi = {10.1038/nrc1886},
isbn = {1474-175X (Print)$\backslash$n1474-175X (Linking)},
issn = {1474-175X},
journal = {Nature reviews. Cancer},
number = {6},
pages = {449--458},
pmid = {16723991},
title = {{Metastasis: a question of life or death.}},
volume = {6},
year = {2006}
}
@article{Mohle:2005,
abstract = {We provide a scaling for compound Poisson distributions that leads (under certain conditions on the Fourier transform) to a weak convergence result as the parameter of the distribution tends to infinity. We show that the limiting probability measure belongs to the class of stable Cauchy laws with Fourier transform t ↦ exp(-c|t|-iat log |t|). We apply this convergence result to the standard discrete Luria-Delbrueck distribution and derive an integral representation for the corresponding limiting density, as an alternative to that found in a closely related paper of Kepler and Oprea. Moreover, we verify local convergence and we derive an integral representation for the distribution function of the limiting continuous Luria-Delbr\{\"{u}\}ck distribution.},
author = {M\"{o}hle, M},
issn = {00219002},
journal = {Journal of Applied Probability},
number = {3},
pages = {pp. 620--631},
publisher = {Applied Probability Trust},
title = {{Convergence Results for Compound Poisson Distributions and Applications to the Standard Luria-Delbr\"{u}ck Distribution}},
url = {http://www.jstor.org/stable/30040845},
volume = {42},
year = {2005}
}

@book{Murray:2002,
abstract = {From reviews of the original edition: "Murray has produced a magnificent compilation of mathematical models and their applications in biology." Nature "Murray's Mathematical Biology belongs on the shelf of any person with a serious interest in mathematical biology." Bulletin of Mathematical Biology SIAM, 2004: "Murray's Mathematical Biology is a classic that belongs on the shelf of any serious student or researcher in the field. Together the two volumes contain well over 1000 references, a rich source of material, together with an excellent index to help readers quickly find key words. ... I recommend the new and expanded third edition to any serious young student interested in mathematical biology who already has a solid basis in applied mathematics." From the reviews of the third edition: "Mathematical Biology would be eminently suitable as a text for a final year undergraduate or postgraduate course in mathematical biology \ldots . It is also a good source of examples for courses in mathematical methods \ldots . Mathematical Biology provides a good way in to the field and a useful reference for those of us already there. It may attract more mathematicians to work in biology by showing them that there is real work to be done." (Peter Saunders, The Mathematical Gazette, Vol. 90 (519), 2006)},
author = {Murray, James D},
booktitle = {Interdisciplinary Applied Mathematics},
isbn = {978-0-387-95223-9},
issn = {0387952233},
publisher = {Springer},
keywords = {Mathematical Biology,Mathematical Models in Biolo},
title = {{Mathematical Biology I. An Introduction}},
volume = {17},
year = {2002}
}


@article{Natarajan:2003,
author = {Natarajan, Loki and Berry, Charles C and Gasche, Christoph},
journal = {Biometrics},
pages = {555--561},
title = {{Estimation of Spontanious Mutation Rates}},
volume = {59},
year = {2003}
}
@article{Newman:2005,
author = {Newman, MEJ},
journal = {Contemporary Physics},
number = {},
pages = {323-351},
title = {{Power laws, Pareto distributions and Zipf's law}},
volume = {46 (5)},
year = {2005}
}
@article{Nithyaja:2009,
author = {Nithyaja, B and Jisha, V.K. and Et al},
journal = {Laser Physics},
number = {3},
pages = {468--472},
title = {{Kinetics of Bacterial Colony Growth by Laser Induced Fluorescence}},
volume = {19},
year = {2009}
}
@book{Nowak:2006,
author = {Nowak, Martin A},
isbn = {0-674-02338-2/hbk},
pages = {xi + 363},
publisher = {Cambridge, MA: The Belknap Press of Havard University Press},
title = {{Evolutionary dynamics. Exploring the equations of life.}},
year = {2006}
}
@book{Olver:2010:NHMF,
      editor = "F.~W.~J. Olver and D.~W. Lozier and R.~F. Boisvert and C.~W. Clark",
       title = "{NIST Handbook of Mathematical Functions}",
   publisher = "Cambridge University Press",
     address = "New York, NY",
        year = "2010",
        note = "Print companion to \cite{NIST:DLMF}"}
                
@article{Pakes:1993,
author = {Pakes, Anthony G},
journal = {Journal of Applied Probability},
number = {4},
pages = {991--994},
title = {{Remarks on the \{L\}uria-\{D\}elbr\"{u}ck Distribution}},
volume = {30},
year = {1993}
}
@article{Prodinger:1996a,
author = {Prodinger, Helmut},
issn = {0021-9002},
journal = {J. Appl. Probab.},
number = {1},
pages = {282--283},
title = {{Asymptotics of the \{L\}uria-\{D\}elbr\{\"{u}\}ck distribution via singularity analysis}},
volume = {33},
year = {1996}
}
@article{Prodinger:1996,
author = {Prodinger, Helmut},
journal = {Journal of Applied Probability},
number = {1},
pages = {282--283},
title = {{Asymptotics of the \{L\}uria-\{D\}elbr\"{u}ck Distribution via Singularity Analysis}},
volume = {33},
year = {1996}
}
@article{Rosche:2000,
author = {Rosche, William A and Foster, Patricia L},
journal = {Methods},
pages = {4--17},
title = {{Determining mutation rates in bacterial populations}},
volume = {20},
year = {2000}
}
@book{Schiff:1999,
abstract = {The Laplace transform is an extremely versatile technique for solving differential equations, both ordinary and partial. It can also be used to solve difference equations. The present text, while mathematically rigorous, is readily accessible to students of either mathematics or engineering. Even the Dirac delta function, which is normally covered in a heuristic fashion, is given a completely justifiable treatment in the context of the Riemann-Stieltjes integral, yet at a level an undergraduate student can appreciate. When it comes to the deepest part of the theory, the Complex Inversion Formula, a knowledge of poles, residues, and contour integration of meromorphic functions is required. To this end, an entire chapter is devoted to the fundamentals of complex analysis. In addition to all the theoretical considerations, there are numerous worked examples drawn from engineering and physics.When applying the Laplace transform, it is important to have a good understanding of the theory underlying it, rather than just a cursory knowledge of its application. This text provides that understanding.},
author = {Schiff, JL},
booktitle = {The Mathematical Gazette},
isbn = {0-387-98698-7},
issn = {00255572},
publisher = {Springer},
number = {502},
pages = {178},
title = {{The Laplace Transform: Theory and Applications}},
volume = {85},
year = {1999}
}
@book{Sedgewick:1995,
abstract = {(From the publicity materials) This book is for students taking either a first-year graduate statistics course or an advanced undergraduate statistics course in psychology. . . . Many topics . . . are elaborated here, such as: the nature of interaction and its interpretation, in terms of theory and response scale transformations; generalized forms of analysis of covariance; extensive coverage of multiple comparison methods; coverage of nonorthogonal designs; and discussion of functional measurement. . . . The book is also equipped with an excellent set of class-tested exercises and answers. (PsycINFO Database Record (c) 2006 APA )},
author = {Sedgewick, Robert and Flajolet, Philippe},
doi = {10.1016/j.entcs.2006.07.011},
edition = {1st},
editor = {Sedgewick:1995},
isbn = {9780321905758},
issn = {15710661},
publisher = {Addison-Wesley Professional},
title = {{An introduction to the analysis of algorithms}},
url = {http://medcontent.metapress.com/index/A65RM03P4874243N.pdf$\backslash$nhttp://books.google.com/books?hl=en\&lr=\&id=P3tCB8Q7mA8C\&oi=fnd\&pg=PT21\&dq=An+introduction+to+the+analysis+of+algorithms\&ots=L3UGRNjuCq\&sig=y8JCF7zZUm2BNBl1NLVGKKFotNQ},
year = {1995}
}

@article{Simon:1955,
author = {Simon, Herbert. A.},
journal = {Biometrika},
pages = {425-440},
title = {{On a class of skew distribution functions}},
volume = {42 (3-4)},
year = {1955}
}
@article{Stewart:1990,
author = {Stewart, F M and Gordon, D M and Levin, B R},
journal = {Genetics},
number = {1},
pages = {175--185},
title = {{Fluctuation analysis: the probability distribution of the number of mutants under different conditions}},
volume = {124},
year = {1990}
}
@article{Tavare:1987,
author = {Tavare, Simon},
file = {:C$\backslash$:/Users/Michael/Google Drive/tumor/branching/tavare87.pdf:pdf},
journal = {Journal of Mathematical Biology},
keywords = {- birth process i,e n e a,l o g y,poisson-dirichlet distribution,population genetics i g},
pages = {161--168},
title = {{The birth process with immigration, and the genealogical structure of large populations}},
volume = {25},
year = {1987}
}
@inbook{Tavare:1989,
author = {Tavare, Simon},
chapter = {3},
pages = {41--56},
publisher = {Princeton University Press},
title = {{Mathematical Evolutionary Theory}},
year = {1989}
}
@article{Tomasetti:2012,
abstract = {In this work, we consider the problem of estimating the probability for a specific random genetic mutation to be present in a tumor of a given size. Previous mathematical models have been based on stochastic methods where the tumor was assumed to be homogeneous and, on average, growing exponentially. In contrast, we are able to obtain analytical results for cases where the exponential growth of cancer has been replaced by other, arguably more realistic types of growth of a heterogeneous tumor cell population. Our main result is that the probability that a given random mutation will be present by the time a tumor reaches a certain size, is independent of the type of curve assumed for the average growth of the tumor, at least for a general class of growth curves. The same is true for the related estimate of the expected number of mutants present in a tumor of a given size, if mutants are indeed present.},
author = {Tomasetti, Cristian},
file = {:C$\backslash$:/Users/Michael/Google Drive/tumor/resistance/tomasetti12.pdf:pdf},
isbn = {0092-8240},
issn = {00928240},
journal = {Bulletin of Mathematical Biology},
keywords = {Branching processes,Drug resistance,Genetic mutations,Ordinary differential equations,Stem cells,Tumor growth},
number = {6},
pages = {1379--1395},
pmid = {22311065},
title = {{On the probability of random genetic mutations for various types of tumor growth}},
volume = {74},
year = {2012}
}
@article{Vogelstein:2013,
author = {Vogelstein, Bert and Papadopoulos, Nickolas and Velculescu, Victor E and Zhou, Shibin and Diaz, Luis A and Kinzler, Kenneth W},
issn = {00368075},
journal = {Science},
number = {6127},
pages = {pp. 1546--1558},
publisher = {American Association for the Advancement of Science},
series = {New Series},
title = {{Cancer Genome Landscapes}},
url = {http://www.jstor.org/stable/41942080},
volume = {339},
year = {2013}
}
@misc{Weisstein:2015,
author = {Weisstein, Eric W.},
title = {{``Polylogarithm." MathWorld-A Wolfram Web Resource}},
url = {http. http://mathworld.wolfram.com/Polylogarithm.html},
urldate = {2016-01-12},
year={2016}
}

@article{Williams:2016,
author = {Williams, Marc J. and Werner, Benjamin and Barnes, Chris P. and Graham, Trevor A. and Sottoriva, Andrea},
journal = {Nature Genetics},
pages = {238-244},
title = {{Identification of neutral tumor evolution across cancer types}},
volume = {48},
year = {2016}
}

@article{Yachida:2010,
abstract = {Metastasis, the dissemination and growth of neoplastic cells in an organ distinct from that in which they originated, is the most common cause of death in cancer patients. This is particularly true for pancreatic cancers, where most patients are diagnosed with metastatic disease and few show a sustained response to chemotherapy or radiation therapy. Whether the dismal prognosis of patients with pancreatic cancer compared to patients with other types of cancer is a result of late diagnosis or early dissemination of disease to distant organs is not known. Here we rely on data generated by sequencing the genomes of seven pancreatic cancer metastases to evaluate the clonal relationships among primary and metastatic cancers. We find that clonal populations that give rise to distant metastases are represented within the primary carcinoma, but these clones are genetically evolved from the original parental, non-metastatic clone. Thus, genetic heterogeneity of metastases reflects that within the primary carcinoma. A quantitative analysis of the timing of the genetic evolution of pancreatic cancer was performed, indicating at least a decade between the occurrence of the initiating mutation and the birth of the parental, non-metastatic founder cell. At least five more years are required for the acquisition of metastatic ability and patients die an average of two years thereafter. These data provide novel insights into the genetic features underlying pancreatic cancer progression and define a broad time window of opportunity for early detection to prevent deaths from metastatic disease.},
author = {Yachida, Shinichi and Jones, Si\^{a}n and Bozic, Ivana and Antal, Tibor and Leary, Rebecca and Fu, Baojin and Kamiyama, Mihoko and Hruban, Ralph H and Eshleman, James R and Nowak, Martin A and Velculescu, Victor E and Kinzler, Kenneth W and Vogelstein, Bert and Iacobuzio-Donahue, Christine A},
isbn = {1476-4687 (Electronic)$\backslash$r0028-0836 (Linking)},
issn = {0028-0836},
journal = {Nature},
number = {7319},
pages = {1114--1117},
pmid = {20981102},
title = {{Distant metastasis occurs late during the genetic evolution of pancreatic cancer.}},
volume = {467},
year = {2010}
}
@article{Ycart:2013,
abstract = {The estimation of mutation rates and relative fitnesses in fluctuation analysis is based on the unrealistic hypothesis that the single-cell times to division are exponentially distributed. Using the classical Luria-Delbr\"{u}ck distribution outside its modelling hypotheses induces an important bias on the estimation of the relative fitness. The model is extended here to any division time distribution. Mutant counts follow a generalization of the Luria-Delbr\"{u}ck distribution, which depends on the mean number of mutations, the relative fitness of normal cells compared to mutants, and the division time distribution of mutant cells. Empirical probability generating function techniques yield precise estimates both of the mean number of mutations and the relative fitness of normal cells compared to mutants. In the case where no information is available on the division time distribution, it is shown that the estimation procedure using constant division times yields more reliable results. Numerical results both on observed and simulated data are reported.},
archivePrefix = {arXiv},
arxivId = {arXiv:1305.3075v3},
author = {Ycart, Bernard},
doi = {10.1371/journal.pone.0080958},
eprint = {arXiv:1305.3075v3},
file = {:C$\backslash$:/Users/Michael/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Ycart - 2013 - Fluctuation analysis Can estimates be trusted.pdf:pdf},
issn = {19326203},
journal = {PLoS ONE},
number = {12},
pmid = {24349026},
title = {{Fluctuation analysis: Can estimates be trusted?}},
volume = {8},
year = {2013}
}
@article{Yule:1925,
author = {Yule, G Udny},
journal = {Philosophical Transactions of the Royal Society of London. Series B, Containing Papers of a Biological Character},
pages = {21--87},
title = {{A Mathematical Theory of Evolution, Based on the Conclusions of Dr. J. C. Willis, F.R.S.}},
volume = {213},
year = {1925}
}
@article{Zheng:2002,
author = {Zheng, Qi},
journal = {Mathematical Biosciences},
pages = {237--252},
title = {{Statistical and algorithmic methods for fluctuation analysis with SALVADOR as an implementation}},
volume = {176},
year = {2002}
}
@article{Zheng:2005a,
author = {Zheng, Qi},
journal = {Genetics},
number = {2},
pages = {861--864},
title = {{Update on Estimation of Mutation Rates Using Data From Fluctuation Experiments}},
volume = {171},
year = {2005}
}
@article{Zheng:1999,
author = {Zheng, Qi},
issn = {0025-5564},
journal = {Mathematical Biosciences},
number = {1--2},
pages = {1--32},
title = {{Progress of a half century in the study of the Luria-Delbr\"{u}ck distribution}},
volume = {162},
year = {1999}
}
@article{Zheng:2005,
author = {Zheng, Qi},
journal = {Mathematical Biosciences},
pages = {198--214},
title = {{New algorithms for Luria-Delbr\"{u}ck fluctutation analysis}},
volume = {196},
year = {2005}
}
@misc{NIST:DLMF,
         key = "{\relax DLMF}",
               year={2016},
       title = "{NIST Digital Library of Mathematical Functions}",
howpublished = "http://dlmf.nist.gov/, Release 1.0.11 of 2016-06-08",
         url = "http://dlmf.nist.gov/",
        note = "Online companion to \cite{Olver:2010:NHMF}"
   }
   
@book{Stein:03,
author = {Stein, Elias M. and Shakarchi, Rami},
publisher = {Princeton University Press},
title = {{Complex Analysis}},
year = {2003}
}

